Four Sub-Saturns with Dissimilar Densities: Windows into Planetary Cores and Envelopes

We present results from a Keck/HIRES radial velocity campaign to study four sub-Saturn-sized planets, K2-27b, K2-32b, K2-39b, and K2-108b, with the goal of understanding their masses, orbits, and heavy element enrichment. The planets have similar sizes $(R_P = 4.5-5.5~R_E)$, but have dissimilar masses $(M_P = 16-60~M_E)$, implying a diversity in their core and envelope masses. K2-32b is the least massive $(M_P = 16.5 \pm 2.7~M_E)$ and orbits in close proximity to two sub-Neptunes near a 3:2:1 period commensurability. K2-27b and K2-39b are significantly more massive at $M_P = 30.9 \pm 4.6~M_E$ and $M_P = 39.8 \pm 4.4~M_E$, respectively, and show no signs of additional planets. K2-108b is the most massive at $M_P = 59.4 \pm 4.4~M_E$, implying a large reservoir of heavy elements of about $\approx50~M_E$. Sub-Saturns as a population have a large diversity in planet mass at a given size. They exhibit remarkably little correlation between mass and size; sub-Saturns range from $\approx 6-60~M_E$, regardless of size. We find a strong correlation between planet mass and host star metallicity, suggesting that metal-rich disks form more massive planet cores. The most massive sub-Saturns tend to lack detected companions and have moderately eccentric orbits, perhaps as a result of a previous epoch of dynamical instability. Finally, we observe only a weak correlation between the planet envelope fraction and present-day equilibrium temperature, suggesting that photo-evaporation does not play a dominant role in determining the amount of gas sub-Saturns accrete from their protoplanetary disks.

==> tab_rv.tex <==
% starname, tel, time, mnvel, errvel 
K2-27 & HIRES & 2457059.023437 & -3.30 & 3.58 \\
K2-27 & HIRES & 2457061.126221 & 7.77 & 2.38 \\
K2-27 & HIRES & 2457062.076956 & 9.38 & 1.71 \\
K2-27 & HIRES & 2457412.040041 & -9.22 & 1.98 \\
K2-27 & HIRES & 2457412.993666 & -2.70 & 2.01 \\
K2-27 & HIRES & 2457423.055308 & -8.75 & 1.80 \\
K2-27 & HIRES & 2457439.987851 & -9.38 & 1.99 \\
K2-27 & HIRES & 2457520.804635 & -8.27 & 1.67 \\
K2-27 & HIRES & 2457555.852216 & 2.68 & 2.02 \\
K2-27 & HIRES & 2457562.772437 & 11.21 & 1.84 \\
K2-27 & HIRES & 2457582.776117 & 1.98 & 1.68 \\
K2-27 & HIRES & 2457583.774146 & 12.50 & 1.76 \\
K2-27 & HIRES & 2457584.770613 & -8.72 & 1.88 \\
K2-27 & HIRES & 2457585.775865 & -13.18 & 2.07 \\
K2-27 & HIRES & 2457586.771953 & -15.02 & 2.02 \\
K2-27 & HARPS & 2457187.504940 & -37782.19 & 2.56 \\
K2-27 & HARPS & 2457188.509910 & -37781.64 & 3.49 \\
K2-27 & HARPS & 2457189.541840 & -37771.12 & 2.49 \\
K2-27 & HARPS & 2457190.542310 & -37762.44 & 2.40 \\
K2-27 & HARPS & 2457191.562130 & -37764.87 & 3.63 \\
K2-27 & HARPS & 2457192.501660 & -37793.36 & 5.62 \\
K2-27 & HARPS-N & 2457064.713740 & -37785.55 & 6.56 \\
K2-27 & HARPS-N & 2457064.734130 & -37782.51 & 6.60 \\
K2-27 & HARPS-N & 2457091.586040 & -37808.60 & 10.63 \\
K2-27 & HARPS-N & 2457091.607280 & -37786.84 & 10.57 \\
K2-27 & HARPS-N & 2457092.598130 & -37780.34 & 8.57 \\
K2-27 & HARPS-N & 2457092.619500 & -37785.85 & 8.41 \\
K2-27 & HARPS-N & 2457093.630910 & -37778.34 & 7.21 \\
K2-27 & HARPS-N & 2457093.652450 & -37774.96 & 7.61 \\
K2-27 & HARPS-N & 2457094.593990 & -37773.65 & 6.80 \\
K2-27 & HARPS-N & 2457094.614980 & -37776.59 & 6.86 \\
K2-27 & HARPS-N & 2457096.659190 & -37776.72 & 5.79 \\
K2-27 & HARPS-N & 2457096.680580 & -37750.40 & 7.05 \\
K2-27 & HARPS-N & 2457097.582510 & -37773.44 & 5.36 \\
K2-27 & HARPS-N & 2457097.605530 & -37766.41 & 3.48 \\
K2-27 & HARPS-N & 2457098.589350 & -37781.28 & 2.28 \\
K2-27 & HARPS-N & 2457098.610550 & -37784.85 & 2.55 \\
K2-27 & HARPS-N & 2457098.631670 & -37781.02 & 2.25 \\
K2-27 & HARPS-N & 2457099.583130 & -37775.37 & 3.77 \\
K2-27 & HARPS-N & 2457099.604440 & -37774.54 & 3.57 \\
K2-27 & FIES & 2457045.607900 & -38039.00 & 11.10 \\
K2-27 & FIES & 2457049.657850 & -37953.40 & 22.10 \\
K2-27 & FIES & 2457050.753890 & -37950.90 & 22.80 \\
K2-27 & FIES & 2457051.655560 & -37972.90 & 7.60 \\
K2-27 & FIES & 2457052.791790 & -37995.40 & 35.70 \\
K2-27 & FIES & 2457054.804290 & -37974.40 & 19.00 \\
K2-32 & HIRES & 2457179.918605 & 2.24 & 1.81 \\
K2-32 & HIRES & 2457197.794461 & -3.58 & 1.66 \\
K2-32 & HIRES & 2457199.862032 & -4.57 & 1.79 \\
K2-32 & HIRES & 2457206.923418 & -4.96 & 2.01 \\
K2-32 & HIRES & 2457208.895178 & -2.80 & 1.68 \\
K2-32 & HIRES & 2457211.844938 & -2.49 & 1.71 \\
K2-32 & HIRES & 2457213.943981 & 1.86 & 1.84 \\
K2-32 & HIRES & 2457228.868515 & -3.80 & 1.71 \\
K2-32 & HIRES & 2457245.822754 & -4.84 & 1.64 \\
K2-32 & HIRES & 2457255.794464 & -6.88 & 1.79 \\
K2-32 & HIRES & 2457265.780260 & -5.92 & 1.78 \\
K2-32 & HIRES & 2457290.774116 & -4.75 & 2.07 \\
K2-32 & HIRES & 2457298.738091 & -15.48 & 1.72 \\
K2-32 & HIRES & 2457520.957134 & 2.08 & 1.63 \\
K2-32 & HIRES & 2457555.932942 & 5.91 & 2.00 \\
K2-32 & HIRES & 2457562.002861 & 0.81 & 1.90 \\
K2-32 & HIRES & 2457562.889918 & 1.92 & 1.85 \\
K2-32 & HIRES & 2457577.783201 & -6.38 & 1.72 \\
K2-32 & HIRES & 2457579.858678 & 3.02 & 1.84 \\
K2-32 & HIRES & 2457580.979251 & 6.30 & 1.77 \\
K2-32 & HIRES & 2457581.967955 & 2.65 & 1.88 \\
K2-32 & HIRES & 2457582.847926 & 1.58 & 1.64 \\
K2-32 & HIRES & 2457591.964435 & 3.75 & 1.95 \\
K2-32 & HIRES & 2457595.857889 & -0.40 & 1.89 \\
K2-32 & HIRES & 2457598.907561 & 10.05 & 1.76 \\
K2-32 & HIRES & 2457599.897252 & 0.80 & 1.75 \\
K2-32 & HIRES & 2457615.802408 & -6.52 & 1.71 \\
K2-32 & HIRES & 2457616.798520 & -1.33 & 1.68 \\
K2-32 & HIRES & 2457617.794666 & 12.13 & 1.71 \\
K2-32 & HIRES & 2457618.776553 & 0.63 & 1.64 \\
K2-32 & HIRES & 2457620.799396 & 1.58 & 1.72 \\
K2-32 & HARPS & 2457185.606900 & 10.69 & 2.65 \\
K2-32 & HARPS & 2457185.677180 & 10.92 & 2.34 \\
K2-32 & HARPS & 2457185.819740 & 9.38 & 2.73 \\
K2-32 & HARPS & 2457185.849750 & 3.16 & 4.14 \\
K2-32 & HARPS & 2457186.599740 & 1.56 & 3.49 \\
K2-32 & HARPS & 2457186.669810 & 8.09 & 2.97 \\
K2-32 & HARPS & 2457186.790150 & 0.48 & 2.84 \\
K2-32 & HARPS & 2457186.823630 & 6.96 & 3.18 \\
K2-32 & HARPS & 2457187.674590 & 5.04 & 1.66 \\
K2-32 & HARPS & 2457187.743820 & 2.94 & 2.41 \\
K2-32 & HARPS & 2457187.781380 & 0.31 & 2.22 \\
K2-32 & HARPS & 2457187.815060 & 8.21 & 3.13 \\
K2-32 & HARPS & 2457188.638490 & 6.46 & 2.19 \\
K2-32 & HARPS & 2457188.694030 & 5.69 & 1.73 \\
K2-32 & HARPS & 2457188.759580 & -8.45 & 3.83 \\
K2-32 & HARPS & 2457188.799060 & -1.28 & 2.62 \\
K2-32 & HARPS & 2457188.831410 & 10.79 & 3.66 \\
K2-32 & HARPS & 2457189.641080 & -1.58 & 2.19 \\
K2-32 & HARPS & 2457189.698560 & -1.46 & 1.71 \\
K2-32 & HARPS & 2457189.756430 & -3.27 & 1.53 \\
K2-32 & HARPS & 2457189.788900 & -8.02 & 1.53 \\
K2-32 & HARPS & 2457189.822940 & -8.48 & 1.78 \\
K2-32 & HARPS & 2457190.649150 & -6.05 & 1.67 \\
K2-32 & HARPS & 2457190.684000 & -2.64 & 1.73 \\
K2-32 & HARPS & 2457190.717160 & -7.75 & 2.04 \\
K2-32 & HARPS & 2457190.749880 & -3.93 & 2.18 \\
K2-32 & HARPS & 2457190.784200 & -8.97 & 2.22 \\
K2-32 & HARPS & 2457191.668780 & -10.48 & 3.27 \\
K2-32 & HARPS & 2457191.706420 & -13.28 & 2.14 \\
K2-32 & HARPS & 2457191.760950 & -4.02 & 2.42 \\
K2-32 & HARPS & 2457191.794930 & -4.92 & 3.20 \\
K2-32 & HARPS & 2457191.824910 & -0.74 & 3.98 \\
K2-32 & HARPS & 2457192.659640 & -2.13 & 3.69 \\
K2-32 & HARPS & 2457198.721430 & -2.16 & 4.51 \\
K2-32 & HARPS & 2457198.809820 & -11.76 & 2.74 \\
K2-32 & HARPS & 2457199.601360 & -9.32 & 1.89 \\
K2-32 & HARPS & 2457199.683460 & -13.58 & 1.59 \\
K2-32 & HARPS & 2457211.700080 & 11.06 & 2.31 \\
K2-32 & HARPS & 2457253.485430 & -0.60 & 2.50 \\
K2-32 & HARPS & 2457264.518160 & 6.03 & 2.99 \\
K2-32 & HARPS & 2457267.563880 & 15.81 & 2.15 \\
K2-32 & HARPS & 2457270.501470 & -0.73 & 1.92 \\
K2-32 & HARPS & 2457278.568590 & 12.00 & 3.48 \\
K2-32 & PFS & 2457198.674600 & -13.95 & 2.31 \\
K2-32 & PFS & 2457199.745540 & -24.28 & 2.56 \\
K2-32 & PFS & 2457200.687220 & -12.24 & 2.16 \\
K2-32 & PFS & 2457204.724130 & 0.00 & 2.40 \\
K2-32 & PFS & 2457205.640810 & 2.07 & 2.09 \\
K2-32 & PFS & 2457206.669050 & 2.37 & 2.67 \\
K2-39 & HIRES & 2457245.118029 & -2.77 & 1.84 \\
K2-39 & HIRES & 2457247.115704 & 20.95 & 1.98 \\
K2-39 & HIRES & 2457254.096811 & 5.63 & 1.73 \\
K2-39 & HIRES & 2457255.116237 & 12.80 & 1.88 \\
K2-39 & HIRES & 2457256.114561 & 21.77 & 1.98 \\
K2-39 & HIRES & 2457285.972002 & -13.26 & 2.12 \\
K2-39 & HIRES & 2457294.966501 & -7.51 & 1.92 \\
K2-39 & HIRES & 2457297.004163 & -6.29 & 1.83 \\
K2-39 & HIRES & 2457298.996728 & -23.50 & 1.99 \\
K2-39 & HIRES & 2457326.887569 & -20.17 & 1.84 \\
K2-39 & HIRES & 2457353.832919 & -18.41 & 1.93 \\
K2-39 & HIRES & 2457354.795982 & -33.97 & 1.85 \\
K2-39 & HIRES & 2457355.815810 & -34.95 & 1.83 \\
K2-39 & HIRES & 2457384.699690 & 15.63 & 1.88 \\
K2-39 & HIRES & 2457401.701268 & -9.00 & 2.08 \\
K2-39 & HIRES & 2457411.706541 & -7.60 & 1.89 \\
K2-39 & HIRES & 2457412.703813 & 4.93 & 2.01 \\
K2-39 & HIRES & 2457413.701618 & -8.03 & 2.27 \\
K2-39 & HIRES & 2457414.703453 & -19.32 & 2.73 \\
K2-39 & HIRES & 2457556.086190 & 17.44 & 2.02 \\
K2-39 & HIRES & 2457562.115673 & -4.76 & 1.91 \\
K2-39 & HIRES & 2457570.091115 & -4.81 & 2.55 \\
K2-39 & HIRES & 2457571.084958 & -16.43 & 2.26 \\
K2-39 & HIRES & 2457580.067841 & 3.69 & 1.83 \\
K2-39 & HIRES & 2457581.053491 & 4.03 & 1.80 \\
K2-39 & HIRES & 2457582.050899 & 7.86 & 1.80 \\
K2-39 & HIRES & 2457583.068181 & 21.20 & 1.84 \\
K2-39 & HIRES & 2457584.045077 & 18.69 & 1.86 \\
K2-39 & HIRES & 2457584.934292 & -6.27 & 1.80 \\
K2-39 & HIRES & 2457586.034712 & -1.41 & 1.87 \\
K2-39 & HIRES & 2457587.004382 & 20.57 & 1.73 \\
K2-39 & HIRES & 2457588.004041 & 15.72 & 1.82 \\
K2-39 & HIRES & 2457595.931932 & -5.51 & 1.94 \\
K2-39 & HIRES & 2457597.041110 & 8.10 & 2.24 \\
K2-39 & HIRES & 2457597.989850 & -7.75 & 1.95 \\
K2-39 & HIRES & 2457599.000004 & -11.60 & 1.88 \\
K2-39 & HIRES & 2457600.028213 & 1.02 & 1.76 \\
K2-39 & HIRES & 2457600.989751 & 6.10 & 2.00 \\
K2-39 & HIRES & 2457602.085344 & 17.36 & 1.75 \\
K2-39 & HIRES & 2457615.880284 & 6.35 & 1.98 \\
K2-39 & HIRES & 2457616.903269 & -2.08 & 1.88 \\
K2-39 & HIRES & 2457622.014940 & -10.94 & 2.04 \\
K2-39 & HARPS & 2457255.714330 & 24507.93 & 2.66 \\
K2-39 & HARPS & 2457256.659920 & 24505.27 & 2.62 \\
K2-39 & HARPS & 2457257.783490 & 24485.83 & 1.31 \\
K2-39 & HARPS & 2457258.704380 & 24462.17 & 2.40 \\
K2-39 & HARPS & 2457260.710270 & 24501.40 & 2.28 \\
K2-39 & HARPS & 2457276.755570 & 24473.82 & 3.85 \\
K2-39 & HARPS & 2457278.749390 & 24500.67 & 1.88 \\
K2-39 & PFS & 2457257.799090 & 0.73 & 1.64 \\
K2-39 & PFS & 2457258.774520 & -9.97 & 1.57 \\
K2-39 & PFS & 2457261.805230 & 0.00 & 1.46 \\
K2-39 & PFS & 2457267.702400 & -20.64 & 1.40 \\
K2-39 & PFS & 2457268.783070 & -5.45 & 1.51 \\
K2-39 & PFS & 2457269.725280 & 14.95 & 1.54 \\
K2-39 & FIES & 2457235.669620 & 24557.22 & 6.99 \\
K2-39 & FIES & 2457239.502420 & 24580.43 & 5.65 \\
K2-39 & FIES & 2457239.572520 & 24582.36 & 5.52 \\
K2-39 & FIES & 2457239.653830 & 24576.87 & 6.13 \\
K2-39 & FIES & 2457240.518660 & 24581.82 & 4.81 \\
K2-39 & FIES & 2457240.624750 & 24575.68 & 5.84 \\
K2-39 & FIES & 2457241.551600 & 24590.82 & 7.26 \\
K2-39 & FIES & 2457241.645910 & 24595.43 & 5.24 \\
K2-39 & FIES & 2457248.678380 & 24565.10 & 18.44 \\
K2-39 & FIES & 2457249.583120 & 24575.34 & 6.52 \\
K2-39 & FIES & 2457261.533170 & 24577.38 & 6.00 \\
K2-39 & FIES & 2457262.666620 & 24554.68 & 7.26 \\
K2-39 & FIES & 2457342.429530 & 24539.24 & 6.00 \\
K2-39 & FIES & 2457343.420360 & 24556.29 & 9.07 \\
K2-39 & FIES & 2457344.411330 & 24544.61 & 7.31 \\
K2-39 & FIES & 2457394.326830 & 24583.37 & 5.60 \\
K2-39 & FIES & 2457395.319990 & 24581.37 & 5.30 \\

